How Long to Estimate Sparse MIMO Channels

Large MIMO transceivers are integral components of next-generation wireless networks. However, for such systems to be practical, their channel estimation process needs to be fast and reliable. Although several solutions for fast estimation of sparse channels do exist, there is still a gap in understanding the fundamental limits governing this problem. Specifically, we need to better understand the lower bound on the number of measurements under which accurate channel estimates can be obtained. This work bridges that knowledge gap by deriving a tight asymptotic lower bound on the number of measurements. This not only helps develop a better understanding for the sparse MIMO channel estimation problem, but it also provides a benchmark for evaluating current and future solutions.

==> text/mStar.tex <==
%Fix $\delta \in \left( 0 , 1 \right)$ and consider matrices $\boldsymbol{G} \in \mathbb{R}^{m{\times}n}$.
%Suppose there exists $m^{\ast}_{\delta} < n$ such that there does not exist any $\boldsymbol{G}$ whose number of rows $m = m^{\ast}_{\delta}$ which satisfies the RIP property with order $k$ and constant $\delta$. Then, there does not exist any matrix $\boldsymbol{G}$ with number of rows $m < m^{\ast}_{\delta}$ that satisfies the RIP property of order $k$ and constant $\delta$.

\begin{proof}
We will show that there exists a non-trivial lower bound on $m_s$ (i.e., $m^* \neq 0$).
Suppose that $m_s \leq k - 1$. Then, there exists a vector $\boldsymbol{x} \in \mathbb{R}^{n_s}$, with $\norm{\boldsymbol{x}}_0 = k$ such that $\boldsymbol{M_s}\boldsymbol{x} = \boldsymbol{0} < (1-\delta_k^{(s)}) \norm{\boldsymbol{x}}^2$. This follows because any $k$ columns of $\boldsymbol{M_s}$ (whose lengths are $\leq k-1$) are linearly dependent. Therefore, we have that $m^* \geq k$.
Next, we will show that if there exists a matrix $\boldsymbol{M_{s1}}$ which satisfies RIP with order $k$ and constant $\delta_k^{(s)}$, then there also exists a matrix $\boldsymbol{M_{s2}} \in \mathbb{R}^{(m_s+1)\times n_s}$ which also satisfies RIP of order $k$ and constant $\delta_k^{(s)}$.
Simply, construct $\boldsymbol{M_{s2}}$ by adding a zero row to $\boldsymbol{M_{s1}}$. Thus, we have $\norm{\boldsymbol{M_{s1}} \boldsymbol{x}} = \norm{\boldsymbol{M_{s2}} \boldsymbol{x}}$ for any vector $\boldsymbol{x} \in \mathbb{R}^{n_s}$. Hence, $\boldsymbol{M_{s2}}$ also satisfies RIP with order $k$ and constant $\delta_k^{(s)}$. This concludes part (i).

To show that $m^*$ is non-increasing in $\delta_k^{s}$ (part (ii)), define $m^*_{\delta}$ as the solution for the following optimization problem
%\begin{mini!}|l|[2]
%{\substack{\boldsymbol{M}\in \mathbb{R}^{m \times n}}}
%         {m} {}{}
%\addConstraint{ \small (1 {-} \delta) \norm{\boldsymbol{x}}_2^2 \leq \norm{\boldsymbol{M}\boldsymbol{x}}_2^2 \leq (1 {+} \delta) \norm{\boldsymbol{x}}_2^2 }{} \label{eq:constraint}
%\addConstraint{\quad \forall \boldsymbol{x} \in \mathbb{R}^n : \norm{\boldsymbol{x}}_0 = k }{}{} \nonumber
%\end{mini!}
\begin{mini!}|l|[2]
{\substack{\boldsymbol{M_s}\in \mathbb{R}^{m_s \times n_s}}}
         {m_s} {}{}
\addConstraint{ \small \boldsymbol{M_s} \in \mathcal{F}_{\delta}}{}
\end{mini!} 
where $\mathcal{F}_{\delta}$, i.e., the feasible set, is defined as
\begin{align*}
\mathcal{F}_{\delta} \triangleq \{
\boldsymbol{M_s} \in \mathbb{R}^{m_s \times n_s} :&
(1 {-} \delta) \norm{\boldsymbol{x}}_2^2 \leq \norm{\boldsymbol{M}\boldsymbol{x}}_2^2 \leq (1 {+} \delta) \norm{\boldsymbol{x}}^2_2 , \\ &\forall \boldsymbol{x} \in \mathbb{R}^{n_s} : \norm{\boldsymbol{x}}_0 = k 
\}
\end{align*}
Now consider $0 < \delta_1 \leq \delta_2 < 1$. Then, we have $\mathcal{F}_{\delta_1} \subseteq \mathcal{F}_{\delta_2}$, which implies that $m^*_{\delta_1} \geq m^*_{\delta_2}$ since the feasible set of the problem under $\delta_1$ is a subset of that of $\delta_2$.
Finally, part (iii) follows by constructing a function $g(n_s,k,\delta_k^{(s)})$ equal to $m^*$ (and possibly removing any constants).
\end{proof}

==> text/unitary_kronecker.tex <==
To extend this result to the matrix $\boldsymbol{G_v} = \left( \boldsymbol{F}^T \otimes \boldsymbol{W}^H \right)
\left( \boldsymbol{U}_{\boldsymbol{t}}^T \otimes \boldsymbol{U}^H_{\boldsymbol{r}} \right)$, we use the following property
\begin{lemma}
The matrix $\boldsymbol{U} = \boldsymbol{U}_{\boldsymbol{t}}^T \otimes \boldsymbol{U}^H_{\boldsymbol{r}}$ is Unitary
\end{lemma}
\begin{proof}
Let us write the matrix $\boldsymbol{U}$ as the following block matrix
\begin{equation}
\footnotesize
\boldsymbol{U} = \frac{1}{\sqrt{n_t}}
\begin{pmatrix}
\boldsymbol{U}_r^H & \boldsymbol{U}_r^H & \dots & \boldsymbol{U}_r^H \\
\boldsymbol{U}_r^H & e^{-j2\pi \Delta_t \frac{1}{L_t}} \boldsymbol{U}_r^H & \dots & e^{-j2\pi (n_t-1) \Delta_t \frac{1}{L_t}} \boldsymbol{U}_r^H \\
\vdots & \vdots & \ddots & \vdots \\
\boldsymbol{U}_r^H & e^{-j2\pi \Delta_t \frac{n_t-1}{L_t}} \boldsymbol{U}_r^H & \dots & e^{-j2\pi (n_t-1) \Delta_t \frac{n_t-1}{L_t}} \boldsymbol{U}_r^H \\
\end{pmatrix}
\end{equation}
To show that $\boldsymbol{U}$ is unitary, we need to show that $\boldsymbol{U}^H \boldsymbol{U} = \boldsymbol{I}$.
Define $\boldsymbol{M}_{i,j}$ to be the matrix which constitutes the block at row $i$ and column $j$ of $\boldsymbol{U}^H \boldsymbol{U}$.
To show that $\boldsymbol{U}^H \boldsymbol{U}$ is the Identity matrix $\boldsymbol{I}$, we need to show that 
\begin{equation}
\boldsymbol{M}_{i,j} = 
\begin{cases}
\boldsymbol{I} & \text{if} \quad i = j \\
\boldsymbol{0} & \text{if} \quad i \neq j
\end{cases}
\end{equation}
We can derive $\boldsymbol{M}_{i,j}$ to be as follows:
\begin{align}
\boldsymbol{M}_{i,j} 
&= \frac{1}{n_t} \sum_{k = 0}^{n_t-1} \left( e^{j 2 \pi (i-1) \Delta_t \frac{k}{L_t}} \boldsymbol{U_r} \right) \left( e^{-j2\pi (j-1) \Delta_t \frac{k}{L_t}} \boldsymbol{U}_{\boldsymbol{r}}^H \right) \nonumber \\
&=  \frac{1}{n_t} \boldsymbol{U_r} \boldsymbol{U}_{\boldsymbol{r}}^H \sum_{k = 0}^{n_t-1}  e^{j 2 \pi (i-j) \frac{k}{n_t}}
\end{align}

We can write the
\end{proof}
\begin{lemma}[Corollary 13 in \cite{broxson2006kronecker}]
If $\boldsymbol{M_1}$ and $\boldsymbol{M_2}$ are unitary matrices, then $\boldsymbol{M} = \boldsymbol{M_1} \otimes \boldsymbol{M_2}$ is a unitary matrix.
\end{lemma}
This shows that the matrix $\boldsymbol{U}_{\boldsymbol{t}}^T \otimes \boldsymbol{U}^H_{\boldsymbol{r}}$ is unitary since both $\boldsymbol{U}_{\boldsymbol{t}}^T$ and $\boldsymbol{U}^H_{\boldsymbol{r}}$ are unitary DFT matrices.
Finally, \cite{eldar2012compressed} claims that there exists constructions for sensing matrices such that the multiplication with Unitary matrices does not affect the distribution of its coefficients, e.g., Gaussian distributed coefficient.
Hence, the bound we obtain in Eq. (\ref{eq:CS_lowerBoundMIMO_tight}) is tight.


